Cardiac Cohort Classification based on Morphologic and Hemodynamic Parameters extracted from 4D PC-MRI Data

An accurate assessment of the cardiovascular system and prediction of cardiovascular diseases (CVDs) are crucial. Measured cardiac blood flow data provide insights about patient-specific hemodynamics, where many specialized techniques have been developed for the visual exploration of such data sets to better understand the influence of morphological and hemodynamic conditions on CVDs. However, there is a lack of machine learning approaches techniques that allow a feature-based classification of heart-healthy people and patients with CVDs. In this work, we investigate the potential of morphological and hemodynamic characteristics, extracted from measured blood flow data in the aorta, for the classification of heart-healthy volunteers and patients with bicuspid aortic valve (BAV). Furthermore, we research if there are characteristic features to classify male and female as well as older heart-healthy volunteers and BAV patients. We propose a data analysis pipeline for the classification of the cardiac status, encompassing feature selection, model training and hyperparameter tuning. In our experiments, we use several feature selection methods and classification algorithms to train separate models for the healthy subgroups and BAV patients. We report on classification performance and investigate the predictive power of morphological and hemodynamic features with regard to the classification of the defined groups. Finally, we identify the key features for the best models.

==> Cardiac Cohort Classification based 4D PC-MRI Data/Sections/01_Introduction.tex <==
% \todo[inline,caption={}]{
% General reviewer remarks:
% \begin{itemize}
%     \item I think the title could be more specific since the paper deals with BAV which is not as general as the title suggest. \textcolor{red}{Wir lassen den Titel so wie er jetzt ist.}
%     % Classification of Biscupid Aortic Valve Patients based on Morphologic and Hemodynamic Parameters extracted from 4D PC-MRI Data
%     \item It would be good to make clear how BAV is diagnosed now and whether there are problems with it.
%     \item It would be good to mention how many features are there initially and how many are being removed at each step.
% \end{itemize}
% }
\section{Introduction}
\label{sec:intro}
%% ============================================================================
%% ============================================================================
Worldwide, most people die of cardiovascular diseases (CVDs)~\cite{mendis2011}. 
%% ============================================================================
Therefore, an accurate assessment of the cardiovascular system and prediction 
of CVDs are crucial. 
%% ============================================================================
Various factors influence the formation and progression of CVDs. 
%% ============================================================================
Besides abnormal vascular morphology and genetic factors, there appear to be 
relationships between hemodynamics and cardiac pathologies~\cite{franccois2012,geiger2012,lorenz2014,McNally.2017}.
%% ============================================================================

%% ============================================================================
To investigate these relationships, patient-specific flow information is required. 
%% ============================================================================
In clinical routine, two-dimensional phase-contrast magnetic resonance imaging 
flow measurements (2D PC-MRI) are used for the diagnosis and follow-up of 
cardiovascular diseases. 
%% ============================================================================
They allow the non-invasive quantification of flow volumes, amount of backward flow and peak flow 
velocities and thus an assessment of the severity of heart valve defects and the 
determination of general heart function. 
%% ============================================================================
However, 2D PC-MRI has serious limitations. 
%% ============================================================================
The analysis is limited to the selected single layer and one flow direction. 
%% ============================================================================
Adjacent vessel sections or flow components outside the main flow direction 
cannot be assessed. 
%% ============================================================================
Correct angulation of the measuring plane to the vessel course is essential, as 
angle errors lead to incorrect flow values. 
%% ============================================================================
The flow in the heart vessels, such as the aorta, is a highly complex, time-varying 
3D structure that cannot be completely represented by a single measuring plane and a 
main flow vector. 
%% ============================================================================
In addition, no information about turbulence is obtained. 
%% ============================================================================
This is critical because quantification in the vicinity of turbulence is 
unreliable~\cite{Koehler_2015}.
% ============================================================================

%% ============================================================================
Time-dependent flow data in a 3D volume can be acquired non-invasively using 
four-dimensional phase-contrast magnetic resonance imaging (4D PC-MRI)~\cite{Markl2012}.  
%% ============================================================================
% The data consist of temporally resolved phase and magnitude images in which the 
% flow direction and velocity are coded. 
%% ============================================================================
The flow information can be evaluated in any vessel section with freely 
modifiable measurement planes. 
%% ============================================================================
% In addition, swirls in the blood flow can be visualized and shear forces acting 
% on the vessel wall can be quantified. 
%% ============================================================================
Thus, 4D PC-MRI has great potential to improve the diagnosis, follow-up and 
treatment decisions of CVDs~\cite{Suwa2020}. 
%% ============================================================================

%% ============================================================================
Several groups developed visual exploration techniques for single 
4D PC-MRI data sets~\cite{vanPelt2010, Heiberg2012,Koehler2019,Semaan2014, Wehrum2014} 
involving different flow attributes and solutions for conveying the temporal 
data behavior. 
%% ============================================================================
However, to develop guidelines how to interpret 4D PC-MRI data requires the analysis
of cohorts instead of single data sets. 
%% ============================================================================
Therefore, we study to what extent disease status can be predicted with supervised 
classification models learned on morphological and hemodynamic attributes, which 
were extracted from 4D PC-MRI data of heart-healthy volunteers (HHV) and patients with 
bicuspid aortic valve (BAV). 
%% ============================================================================
To support physicians in diagnosing and assessing the severity of BAV defects 
and to better understand the variety of physiological hemodynamic and morphological 
characteristics, we have formulated three research questions that we aim to answer with 
our classification procedure:  
%% ============================================================================
(i) Do heart-healthy volunteers and BAV patients differ regarding the extracted features~\cite{Ebel2020}?
%% ============================================================================
(ii) Are there predictive features that can separate between older heart-healthy volunteers and BAV patients? 
This question is motivated by the challenge in clinical practice to distinguish between non-pathological decline in cardiac function with increasing age~\cite{Lernfeit1991} (\emph{healthy aging}) and the onset of early stages of BAV, solely based on flow velocity. 
% \smalltodo{- In the introductory section, it is not clear what is the clinical application of the classifier focusing on the second and third hypotheses generated.}
%% ============================================================================
(iii) Do female and male heart-healthy volunteers differ with respect to morphological and hemodynamic attributes? Since women generally have a smaller heart, a smaller blood volume and a faster heartbeat than men~\cite{Legato2004}, the identification of further differences related to aortic blood flow might suggest the necessity to stratify diagnostic procedures or treatment pathways by gender.
%% ============================================================================
% In addition, we investigate if there are characteristic features to classify male 
% and female as well as young and old heart-healthy volunteers. 
%% ============================================================================
We train separate models for the healthy subgroups and BAV patients based on the 
combination of several feature selection methods and learning algorithms. 
%% ============================================================================
Model training is combined with a feature selection step to identify correlations 
between the multitude of flow attributes and to reduce them to a meaningful subset.  
%% ============================================================================
Finally, we study and compare the informativeness of each feature towards the 
outcomes.
%% ============================================================================
Furthermore, the determination of standard values and follow-ups for flow 
attributes is supported. 
%% ============================================================================

==> Cardiac Cohort Classification based 4D PC-MRI Data/Sections/02_RelatedWork.tex <==
\section{Related Work}
\label{sec:relwork}
%% ============================================================================
%% ============================================================================

%% ============================================================================
%% ============================================================================
% Machine learning is frequently used to support computer-aided diagnosis and 
% prediction of heart diseases~\cite{AlAref2019, Dinh2019, Miao2016, Mohan2019, Dolatabadi:SVM2017, Wah2018}. 
There is extensive research on machine learning (ML) in cardiology, for example to support computer-aided diagnosis and prediction of heart diseases~\cite{AlAref2019}. 
% ~\cite{AlAref2019, Dinh2019, Miao2016, Mohan2019, Dolatabadi:SVM2017, Wah2018}. 
%% ============================================================================
Dinh et al.~\cite{Dinh2019} created a classification model ensemble from 
different base classifiers in the context of cardiovascular disease diagnosis.
%% ============================================================================
Patient characteristics such as age, blood pressure, body weight and chest pain 
were found to be most predictive. 
%% ============================================================================
Similarly, Miao et al.~\cite{Miao2016} trained an AdaBoost~\cite{Freund:AdaBoost1997} 
ensemble classifier for coronary heart disease diagnosis using data gathered from 
four different medical institutions. 
%% ============================================================================
Wojnarski et al.~\cite{Wojnarski2018} identified three distinct phenotypes of BAV patients based on vascular morphology via data clustering. 
%% ============================================================================
While acknowledging the high potential of ML, Russak et al.~\cite{Russak2020} observed that case studies of a successful integration of these technologies into clinical practice are still sparse. 
%% ============================================================================
They further suggest guidelines to increase acceptance and ultimately to enable clinical adoption of ML techniques in cardiology, including a project development driven by unsolved clinical questions rather than by the available data only, incorporating experts from multiple disciplines, using complete patient data gathered in a standardized format, improving interpretability of complex ML models, and training clinicians on ML fundamentals to increase familiarity with these concepts. 

%% ============================================================================
Recently, deep learning has become increasingly popular also for cardiovascular applications~\cite{Martin2020, Fries2019, Miao2018, Arabasadi:DL2017, Kim2017}. 
%% ============================================================================
In comparison to classic ML algorithms, deep neural networks often exhibit superior 
accuracy and are able to work on raw image data, thus reducing the necessity to 
carefully extract features using domain knowledge which is often too time-consuming 
or expensive. 
%% ============================================================================
However, the ``black-box'' nature of deep neural networks is rather unsuited for 
inference, which is crucial especially in medical applications. 
%% ============================================================================
Thus, there are studies that create more parsimonious models using extracted 
interpretable parameters to better understand characteristics of anatomical 
structures which are predictive for the outcome. 
%% ============================================================================
Niemann et al.~\cite{Niemann_2018} studied the potential of 22 morphological 
parameters extracted from angiographic images for a data-driven rupture risk 
classification in intracranial aneurysms. 
%% ============================================================================
Post-hoc interpretation steps revealed the most predictive features, which 
included a dome point angle, ellipticity index and aneurysm volume. 
%% ============================================================================
In addition to morphology, Detmer et al.~\cite{Detmer:Neuroradiology2019} investigated 
also hemodynamic parameters and patient characteristics for rupture risk assessment 
and found that ruptured aneurysms exhibit larger and more complex flow characteristics. 
%% ============================================================================

%% ============================================================================
Often, the number of extracted features is large, which often leads to unnecessarily 
complex models. 
%% ============================================================================
Selecting a subset of features can help to reduce computational complexity, 
increase model performance and enhance model interpretability~\cite{Wah2018, Latha2019, Parthiban2008}. 
%% ============================================================================
For example, Latha et al.~\cite{Latha2019} combined ensemble classifiers with a 
preceding feature selection step which improved model accuracy of heart disease prediction.

==> Cardiac Cohort Classification based 4D PC-MRI Data/Sections/03_Preprocessing.tex <==
\section{Medical Background}
\label{sec:dataac}
%% ============================================================================
The vascular system forms an extensive network and, with the heart as the 
central pump, ensures the supply of all organs and tissues with oxygen and vital 
nutrients. 
%% ============================================================================
The aorta is the largest artery in this system.
%% ============================================================================
Their diameter of about 2-3 cm allows the acquisition of a measurable signal for 
a meaningful blood flow analysis.
%% ============================================================================
During systole, oxygenated blood passes from the left ventricle (LV) via the aortic 
valve (AV) into the ascending aorta and is then supplied to the body, see Figure~\ref{fig:heart}.
%% ============================================================================
From the right ventricle, deoxygenated blood is pumped through the pulmonary 
valve into the pulmonary artery.
%% ============================================================================
During diastole, the AV is closed to prevent blood from flowing back into the LV. 
%% ============================================================================
\begin{figure}[t]
   \centering
   \includegraphics[width=0.5\linewidth]{Figures/heart.pdf} %[width=\linewidth]
   \caption{
     \label{fig:heart}
     Anatomy of the human heart.
    }
\end{figure}

\begin{figure*}[t]
  \makebox[\textwidth]{\makebox[1.3\textwidth]{
    \includegraphics[width=1.3\linewidth]{Figures/pipeline.pdf}
  }}
   \caption{
     \label{fig:pipeline}
     \textbf{Schematic overview of our data analysis pipeline.} 
     For each of the 112 4D PC-MRI data sets, we extract morphological and hemodynamic features (197 in total). 
     We build separate classification models on three different subsets. 
     Therefore, we initially split the data into a training set (70\%) and a test set (30\%). 
     Then, we perform feature selection and classifier training. 
     Feature selection hyperparameters are tuned within a 10-fold cross-validation setup. 
     We use a wide range of combinations of feature selection methods and classification algorithms. 
     Finally, we identify the best model that achieves highest performance on the test set.
    }
\end{figure*}

%% ============================================================================
\subsection{BAV and Related Flow Behavior}
\label{subsec:aorticpath}
%% ============================================================================
Hemodynamic characteristics are an indicator for the emergence and progression 
of CVDs. 
%% ============================================================================
Healthy people have only a slight systolic helix in the aortic arch, which 
is considered physiological.
%% ============================================================================
CVDs change the vessel morphology, which increases the probability 
of quantitative and qualitative flow abnormalities~\cite{Kilner1998}.
%% ============================================================================

%% ============================================================================
The bicuspid aortic valve is the most common congenital heart defect with a 
prevalence of 1-2\%~\cite{Ward2000}. 
% ============================================================================
Normally, an aortic valve consists of three leaflets, whereas in a BAV two of them 
are fused together~\cite{Siu2010}. % at different sites 
% ============================================================================
% Due to the faulty morphology of the aortic valve in a BAV patient, two typical 
% secondary diseases often develop over time, \textit{aortic valve stenosis} or 
% \textit{aortic valve insufficiency}. 
Due to the faulty morphology of the aortic valve, 
secondary diseases such as \textit{aortic valve stenosis} or 
\textit{aortic valve insufficiency} often develop over time. 
% ============================================================================
% Both diseases can also occur together. 
% ============================================================================
In aortic valve stenosis, a narrowing of the valve area occurs, so that the 
aortic valve can no longer open completely. 
% ============================================================================
In the case of aortic valve insufficiency, the aortic valve cannot close properly. 
% ============================================================================
As a result, blood in the diastole flows from the aorta back into the left 
ventricle - with the consequence of a volume strain on the left ventricle. 
% ============================================================================
 
% ============================================================================
Several studies investigated the influence of a BAV on flow patterns in the 
ascending aorta~\cite{Hope2010,Meierhofer2013,McNally.2017}. 
% ============================================================================
In comparison with healthy volunteers, patients more often had a helical 
blood flow, often accompanied by an eccentric main blood flow and increased 
wall shear stress. 
% ============================================================================
This results in permanent hemodynamic stress, which can lead to aortic valve 
stenosis, aneurysms, and/or AV insufficiency~\cite{Dux2019}. 
% ============================================================================
Recently, Ebel et al.~\cite{Ebel2020} performed a statistical analysis of 
different flow attributes between healthy and BAV patients, using standard 
techniques such as box plots. 
%% ============================================================================
The greatest differences between the two groups were found in the flow velocities 
and the vortex volume.
%% ============================================================================
However, the cohorts were quite small and there was no computer support for 
attribute selection, which made the analysis process time-consuming and error-prone. 
%% ============================================================================
Thus, a detailed analysis of the flow attributes regarding several cohorts 
remains a challenge. 
% ============================================================================

% ============================================================================
\subsection{Data Acquisition and Feature Extraction}
%% ============================================================================
% \smalltodo{- In Section 3.2, the description of the procedure is not completely clear. First, it looks like the dataset contains a single image in each direction, but then it claims that there are multiple slices. This should be checked.}
A 4D PC-MRI data set contains each three (x-, y- and z-direction)
time-resolved phase and magnitude images that describe the flow direction
and strength, respectively.
%% ============================================================================
All temporal positions together represent one full heartbeat.
%% ============================================================================
A 3 T Siemens Magnetom Verio MR scanner was used with a maximum expected 
velocity ($\text{V}_\text{ENC}$) of 1.5 m/s per dimension.
%% ============================================================================
The spatio-temporal resolution is 1.77 $\times$ 1.77 $\times$ 3.5 mm$^3$ $\backslash$ 
50 ms with a 132 $\times$ 192 grid for each of the 19 to 35 slices and 18 to 33 
time steps.
%% ============================================================================

%% ============================================================================
To analyze individual 4D PC-MRI data sets the software \emph{Bloodline}~\cite{Koehler2019} 
is used, which provides a guided, easy-to-use workflow. 
%% ============================================================================
During pre-processing, phase wraps (aliasing) and magnetic coil artifacts are 
automatically corrected. 
%% ============================================================================
Subsequently, the Graph Cut algorithm is employed to segment individual vessels, 
such as the thoracic aorta or pulmonary artery. 
%% ============================================================================
This results in binary segmentation masks, from which polygonal vessel surfaces 
are extracted using Marching Cubes, which are post-processed by smoothing and reduction. 
%% ============================================================================
In addition, a centerline is determined for each vessel. 
%% ============================================================================
% In addition, six measuring planes are placed semi-automatically at standardized 
% positions~\cite{schulz2013} and aligned orthogonally to the centerlines.
%% ============================================================================

%% ============================================================================
After pre-processing, the complete flow is automatically calculated within the 
vessel based on flow information encoded in the phase images. 
%% ============================================================================
On the one hand, a qualitative analysis is performed to explore patient-specific 
flow patterns such as vortices, which may be an indicator of pathological 
changes~\cite{Hope2010}. 
%% ============================================================================
On the other hand, quantitative methods allow the evaluation of the heart function. 
%% ============================================================================
For this purpose, 197 attributes, such as heart rate, or maximum vessel diameter, 
commonly used in clinical studies, are calculated automatically. 
%% ============================================================================

%% ============================================================================
For the hemodynamic features, a distinction is made between two large groups: 
features that affect the vortical flow and features that describe the laminar flow. 
%% ============================================================================
The proportion of vortical flow was determined using the $\lambda_2$ criterion. 
%% ============================================================================
In addition, planes were placed in the aorta along the centerline. 
%% ============================================================================
For each plane, different properties of the vortical flow were measured over 
the time steps. 
%% ============================================================================
The maximum, minimum, median and mean values per feature were then determined 
for the set of result values over all planes and time steps. 
%% ============================================================================
Since these properties are based on the planes along the aorta, they are also 
called ``in-plane'' features. 
%% ============================================================================
In addition, so-called ``through-plane'' features, which characterize 
the laminar flow, are automatically calculated~\cite{Koehler2019} at specific 
landmarks. 
%% ============================================================================
Subtracting the vortical portion from the total flow, the laminar flow 
portion is obtained. 
%% ============================================================================
Similar to the in-plane features, the through-plane features are determined at 
each plane over time and the maximum, minimum, median and mean value per feature 
is calculated.
%% ============================================================================
% \begin{enumerate}
%     \item \emph{Global, time-independent attributes} (refer to 
%     the entire vessel and do not change during the time of a heartbeat), e.g., 
%     the heart rate, or maximum vessel diameter.
%     \item \emph{Global, time-dependent, attributes}, e.g., maximum velocities or vortex 
%     volumes. Here, the mean within the vessel segmentation is calculated and then 
%     minimum, maximum, mean, and median values are provided for each time step.
% \end{enumerate}
%% ============================================================================
%% ============================================================================
% Moreover, two types of attributes are calculated for each measuring plane:
% %% ============================================================================
% \begin{enumerate}
%     \item \emph{Plane-based, time-independent attributes}, e.g., flow rate or 
%     cardiac output. Here, the mean within the plane is calculated and then minimum, 
%     maximum, mean, and median values are provided for each measuring plane.
%      \item \emph{Plane-based, time-dependent attributes}, e.g., flow rate per time or angle of 
%      the flow jet. Here, for each time step minimum, maximum, mean, and median 
%      values are provided within each measuring plane.
% \end{enumerate}
%% ============================================================================
%% ============================================================================

%% ============================================================================
Finally, all data collected with Bloodline can be exported, enriched with additional 
information about the patient (age, gender, weight, etc.) and recording modalities 
(MRI sequence, recording duration, etc.).
%% ============================================================================
So far, 90 data sets of heart-healthy volunteers and 22 BAV patients have been 
evaluated with Bloodline. 
% \smalltodo{ASK BEN: At the end of Section 3.2, you are giving statements about the patients. Shouldn't the patients with other diseases be discarded, since BAV is related to aorta? Can differences in flow induced by other CVDs affect the features used for the classification?}
%% ============================================================================
These 112 data sets serve as input for our classification pipeline. 
%% ============================================================================
Currently, we focus on the analysis of aortic flow data, as we have 
only few patients with pathological changes in other vessels such as the 
pulmonary artery.
%% ============================================================================
Aortic diseases occur more frequently in clinical routine and are therefore 
our main focus.

==> Cardiac Cohort Classification based 4D PC-MRI Data/Sections/04-1_prepro.tex <==
\subsection{Data Pre-Processing}
As part of data pre-processing, we remove highly correlated and low variance features, with the purpose of mitigating the negative effects caused by multicollinearity, and to prevent building unnecessary complex classification models. 
Ideally, our models achieve highly predictive performance and are as simple as possible at the same time, i.e., they should require only a small number of features. 
The correlation heatmap in Figure~\ref{fig:corplot} reveals 5 larger features subsets with moderate to high pairwise correlation. 
% First, we \smalltodo{- Correlation is used to discard features. This is commonly done, but there is a good chance to remove features that actually make the difference between classes despite being correlated. How much of a problem can this be here? Would it make sense to use other methods like Linear Discriminant analysis to identify whether this makes sense? Why is this step needed given that you will do the feature selection in the next step?
% feature selection techniques applied in Section 4.1 are for the sake of removing redundant and irrelevant features
% here, the focus is on feature-feature correlations opposed to the feature-target correlation methods in Section 4.2
% in other words, the methods in Section 4.1 are independent of the class label - LDA is not
% }
remove highly correlated features using the algorithm of Kuhn and Johnson~\cite{Kuhn2013}. 
For this purpose, we first compute Pearson correlation for each pair of features. 
If a pair of features exhibits an absolute correlation value of 0.9 or higher, we keep the feature that has the lower average correlation with the rest of the features. 
We repeat this process until none of the correlation values exceed the specified threshold.
In the process, we remove 103 of such features. 
Secondly, we eliminate near-constant features, where the most frequent value (rounded to two decimal places for continuous features) occurs more than 20 times as often as the second most frequent value and where the number of unique values is smaller than 10. 
We remove 3 such features, resulting in a total of 94 features for classification. 
% First,
% we determine the pair of attributes with the largest absolute correlation.
% Afterwards, for each of the two attributes, we compute the average pair-
% wise correlation to all other attributes. The attribute with the larger of
% the two values is removed. This process is repeated until all correlation
% values fulfill the speciﬁed range.

% For the second classification task, we use Gender as the target variable and only HVV patients were extracted for classification, to determine if Gender played any role in determining a patient's cardiac health. The initial pre-processing of removal of highly correlated features resulted in 90 features getting removed and 3 features getting removed from the near-zero variance filtering process. 107 features remained for the final classification.

\begin{figure}[htb]
   \centering
   \includegraphics[width=0.5\linewidth]{Figures/corplot.pdf}
   \caption{
     \label{fig:corplot}
     \textbf{Correlation heatmap.} 
     Spearman correlation heatmap for all 200 features (197 morphological and hemodynamic parameters, age, gender, and body weight). 
     Features are ordered by the result of agglomerative hierarchical clustering with complete linkage. 
     Subsets of at least 10 features with moderate to high pairwise correlation are enframed with black squares.
    }
\end{figure}

For the second classification task, we divide the feature ``age'' into two intervals, which we refer to as ``younger'' and ``older'', respectively.
We determine the cutoff value as age with maximum information gain~\cite{Quinlan1986} towards cardiac status (cf. Figure~\ref{fig:histogram-age-distribution}).
% min_group_size = 30 doesn't need to be reported, because it turned out, that 47 is always the best cutoff, independently from a minimum group size
Discretization leads to a subgroup of 78 younger subjects up to and including 
% \smalltodo{How is the threshold of 47 determine and the relation to the hypothesis. Would it not be possible to test for multiple thresholds to see what would be the best performance and actually then define which is the age in which the difference starts to disapear?}
47 years (60 HHV, 18 BAV patients), and a subgroup of 34 older subjects (30 HHV, 4 BAV patients). 
% After removal of 111 highly correlated features and 3 near-zero variance features, 86 features remained for the final classification.
The data was then divided into a training set and a testing set, with a ratio of 70:30 for further analysis.
% The initial stage before any Feature Selection can be accomplished, the 122 data samples alongwith the 200 feature instances needed to be preprocessed in order to make them ready for three different classification tasks. The first step was to eliminate the Label class 3 namely, "Tetralogy of Fallot" as according to the resources this class of patients did not contribute towards the cardiological complexities of a patient after which we were left with 112 data points.
% The second step was to remove the features which are highly correlated to each other in order to remove any bias that may appear which can lead to the overfitting of the data classification model. The features which had a correlation factor of 0.9 or higher were removed. 
% Moreover, there were features which had a near zero variance, i.e., with identical values for the entire feature column. This means that the features do not have any contribution towards the classification task and can be removed. After the removal of all such features, there were in total 95 features over which the classification needs to be performed. Moreover, there were 90 data points with class label "Healthy" and 22 data points with class label "BAV" which means there is high class imbalance in the data which might lead to bias.
% For the classification task of finding whether Gender has a role to play in the patients being Healthy, only data with class label "Healthy" were extracted and again the highly correlated features and features with zero variance were eliminated. Each Gender class had 45 points each and hence were equally distributed.
% Similarly to check if there are any similarities between the flow conditions of Old Healthy patients and BAV patients, we set 47 years as a threshold and extract all Healthy class patients above 47 years(Old Healthy) and all other BAV patients. The main idea behind this was to build a classification model using this data and to check how the model performs. In case the model's performance is not good, it would mean that the model was not able to distinguish between the characteristics of the Old Healthy patients and the BAV patients, resulting in several misclassifications, which verifies the hypothesis that Old Healthy patients have the same flow conditions as BAV patients. The reason the age threshold was set to 47 was for the fact that this particular threshold resulted in the maximum Information Gain towards the classification as well as resulted in the Healthy class having 30 data points which was enough data to proceed with the classification task. 
% The data was then divided into Training and Testing set, with a ratio of 70:30 for further analysis.

\begin{figure}[htb]
   \centering
   \includegraphics[width=0.65\linewidth]{Figures/histogram-age-distribution.pdf}
   \caption{
     \label{fig:histogram-age-distribution}
     \textbf{Age distribution.} 
     According to information gain towards cardiac status, the optimal cutoff for a binary discretization is 47 years (right-closed).  
     We train a separate classification model that distinguishes between heart-healthy volunteers older than 47 years and all BAV patients. 
     Light gray bars show the overall age distribution.
    }
\end{figure}

==> Cardiac Cohort Classification based 4D PC-MRI Data/Sections/04-2_fs.tex <==
\subsection{Feature Selection} %Cardiological Feature Selection
We bundle classifier training with a preceding feature selection step that aims to reduce computational complexity, to increase model performance and enhance model interpretability. 
% Feature Selection is used to select a subset of features that can help reduce the computational complexity of working with data sets with large number of features. These techniques help to find features that contribute the most towards the classification of the data into the label classes or target variables, in our case, "Healthy" and "BAV". Feature Selection methods help improve model performance, enhance interpretability,decrease the training time of the learning process and reduce overfitting of the data to the model by getting rid of redundant features.
Feature selection methods can be broadly categorized into filter and wrapper methods~\cite{Jovic:FSReview2015,Kohavi:WrapperFS1997}.  
Filter methods rank features based on a specific importance measure, e.g., correlation with the target variable. 
The features that were found to be important are kept and then fed to the classification algorithm. 
Typically, the search is performed just once and independent from the classification algorithm. 
In contrast, wrapper methods use the performance of the classification model itself to measure the goodness of a candidate feature subset. 
Traditional wrapper methods work in an iterative, greedy fashion: the model is repeatedly trained on different feature subsets, where model performance on the current feature subset determines which subset to evaluate next. 
We use three filter and four wrapper methods.

\paragraph*{Correlation-based feature selection (CFS) filter} 
The non-parametric CFS~\cite{Hall:CFS2000} searches for a feature subset in which each individual feature is highly correlated towards the target variable but uncorrelated to every other feature within the subset. 
The ``merit'' of a feature is quantified as the quotient between feature-target correlation and feature-feature correlation. 
CFS starts with an empty set and iteratively adds the feature with maximum merit score until none of the remaining feature candidates has a positive merit score.  

\paragraph*{$\chi^2$-test filter}
In statistics, a $\chi^2$-test is used to test the independence of two categorical variables. 
This filter performs a $\chi^2$-test for every feature and the target feature. 
Features are ranked by p-value. 
% Only features that are not independent from the target attributes are kept. % The $\chi^2$ based test was performed by hyperparameter tuning the optimal percentage of features(fw.perc) with highest importance that would result in the maximum performance of the model. The tuning was done for fw.perc with a lower bound of 0 and upper bound of 1 and the optimal fw.perc was used for Testing the model and reporting all performance measures.
Continuous features were discretized beforehand with the non-parametric, supervised method of Fayyad and Irani~\cite{Fayyad:MDL93}. % based on MDL principle
The relative number of features that are retained for classification must be specified. 

\paragraph*{Information gain filter (IG)}
Similarly to the $\chi^2$-test, information gain measures the relationship between the target variable and a feature. 
It is calculated as reduction of uncertainty in the value of the target variable after observing the feature~\cite{Quinlan1986}. 
This filter calculates information gain for every feature with respect to the target variable. 
Just as the $\chi^2$-test, the percentage of selected features must be set.

\paragraph*{Sequential forward search (SFS) wrapper}
SFS is a greedy forward selection method that starts by training a classifier on an empty set of features. 
In each iteration, the feature that improves model performance the most is added to the model. 
If there is no more candidate feature whose addition leads to a relative increase of $\alpha$ in model performance, the method terminates.
% \textcolor{red}{An $\alpha$ value of 0.01 was used as the minimal threshold for improvement.} 

\paragraph*{Sequential backward search (SBS) wrapper} 
SBS follows a search strategy that is reverse to SFS. 
It is a top-down approach which starts training a classifier on the whole feature set and iteratively removes the feature whose elimination leads to the least decrease in model performance.  
If there is no more candidate feature whose removal leads to an relative decrease of less than $\beta$ in model performance, the method terminates.
% \textcolor{orange}{@AN Verify this sentence. Do you really mean improvement?->}\textcolor{red}{A $\beta$ value of -0.001 was used as the minimal threshold for improvement.}

\paragraph*{Genetic search (GS) wrapper} 
GS methods are inspired by evolution processes found in nature. 
They emulate the mechanism of natural selection by iteratively performing so called crossover, mutation, elite selection and insertion operations on an initial set of candidate feature subsets~\cite{Oh:GeneticFS2004}. 
These operations involve adding and removing features from individual candidate subsets, creating new feature subsets by combining and swapping features from pairs or groups of candidate subsets, as well as removing some candidate subsets. 
A fitness function, usually the performance of the classification model, determines the probability of survival of a feature subset candidate for the next iteration. 
All operations include some aspects of randomization to avoid a solution from being stuck at a locally optimal feature set.  
The number of initial candidate feature subsets (``parent population'') and the maximum number of iterations were determined via hyperparameter tuning; 
crossover rate is set to 0.5 and mutation rate is set to 0.05.

% It has been shown that, in contrast to SFS and SBS, the heuristic GS is more likely to arrive at the global optimum~\cite{Holland:1993}.  
% \color{orange}
% The size of the parent population determined by the parameter "mu" was taken as 10, as it was found to have produced the best results. Furthermore, the number of iterations, maxit, conducted was 10. The rest of the parameters were given the default values as follows: 
% \begin{itemize}
%     \item same.resampling.instance = TRUE,
%     \item impute.val = NULL,
%     \item max.features = NA\_integer\_, 
%     \item comma = FALSE, 
%     \item crossover.rate = 0.5,
%     \item mutation.rate = 0.05,
%     \item tune.threshold = FALSE, 
%     \item tune.threshold.args = list(), 
%     \item log.fun = "default"
% \end{itemize}
% @AN: Which parameters were tuned?
% \textcolor{red}{The Genetic Search Algorithm is derived from Charles Darwin's theory of Natural Selection and it's role in finding the best gene-pairs for a chromosome combination. In our problem, each feature is a gene and the subset of features which give the best performance is our desired chromosome. The algorithm does not rank individual features based on the class variable but tries to find the combination of features which results in the optimal performance of the learning model.}

\paragraph*{Random search (RS) wrapper} 
At each iteration, RS creates a feature subset candidate by random sampling from the total feature set. 
The model performance of a candidate set has no influence on the construction of the feature subset candidate of the next iteration. 
The number of iterations is varied and the probability of a feature to be randomly selected is 50\%. 
% siehe Bens VCBM'19 paper sec 2.3 beschreibung GA http://www.vismd.de/lib/exe/fetch.php?media=files:misc:behrendt_2019_vcbm.pdf

% A genetic algorithm (GA) is an optimization tool that is based on concepts of evolution population biology (Mitchell 1998; Haupt, Haupt, and Haupt 1998). These algorithms have been shown to be able to locate the optimal or near-optimal solutions of complex functions (Mandal, Jeff Wu, and Johnson 2006). To effectively find optimal solutions the algorithm mimics the evolutionary process of a population by generating a candidate set of solutions for the optimization problem, allowing the solutions to reproduce and create new solutions (reproduction), and promoting competition to give the most fit solutions (i.e., optimal) the best chance to survive and populate the subsequent generation (natural selection). This process enables GAs harness good solutions over time to make better solutions, and has been shown to converge to an optimization plateau (Holland 1992).

% A GA emulates the evolution process found in nature; it is intended to conduct a search for an optimal solution to a given problem by mimicking natural selection. Several research studies have demonstrated the advantages of the GA in solving high dimensionality and FS problems (Gunal, 2012, Uysal and Gunal, 2014, Tsai et al., 2014, Lei, 2012, Uğuz, 2011). However, time consumption, parameter setting and random selection of the initial solution are the main problems associated with the GA. 


% ) and uses this ranking to subset Features based on certain parameters like an Absolute Number of Features to be selected, a certain Percentage of Features to be selected or all Features with an importance measure greater than or equal to a Threshold are selected. These parameters can also be treated as HyperParameters that can be tuned to obtain the optimal subset of Features which would result in the best accuracy results for the classification. 
% The subset of the Features is then used to fit a model for classification.
% Three Filtering methods were used for the Feature Selection method:
% \begin{enumerate}
%     \item Correlation based Feature Selection
%     \item Chi-Square based Feature Selection
%     \item Information Gain based Feature Selection
% \end{enumerate}

% \textbf{1. Correlation based Feature Selection:} The Correlation based Feature Selection was done based on the Hypothesis that a good subset of features is highly correlated to the output class but is unrelated to each other. The "CFS" method of the Caret library was used to do the same. It uses the Pearson Correlation coefficient which is used as the criteria to increase the ratio of feature-to-label-class correlation to feature-to-feature correlation. The higher the correlation coefficient, the better the subset of Features. 

% \textbf{2. Chi-Square based Feature Selection:} The Chi-Square test is used in Statistics to test the independence of two events occurring together, or in other words, the dependence of the occurrence of the label class in presence of a particular feature. The Chi-Square based Feature Selection method utilizes this test to select the features which have very high dependence with the target classes, "Healthy" and "BAV". The "chi.squared" method from the FSelector library was used to select the subset of relevant features.  

% \textbf{3. Information Gain based Feature Selection:} Information Gain can be used for the Feature Selection process by evaluating the mutual information shared between a feature variable and the target variable. The more the information shared between the variables, the more the decrease in entropy of the overall classification, hence, the better the classification. The "information.gain" method of the FSelectorRcpp library was used to select the features with the most information gain with the target variable.  

% The features are extracted from the filter methods, along with the optimal percentage of the features that results in the classification model giving the best results. These features along with the optimal percentage(as a hyperparameter) are then fed to a classification model for training and testing.

% \subsubsection{Wrapper Methods}
% In Filter Methods, the features were selected independent of the classifier model or learning algorithm. Wrapper models on the other hand, utilize the performance of a learning algorithm, to assess the usefulness of a feature subset. The model is trained again and again with various subsets of features and the subset which gives the beat performance in the model is selected.
% Like the hyperparameters of optimal percentage or absolute number of features to be selected for Filter methods, there are certain parameters that are to be selected for the Wrapper Methods as wee, which are:
% \begin{itemize}
%     \item Performance Measures: which performance measures(mean, accuracy, kappa, gmean etc.) needs to be minimized/maximized to assess the usefulness of the features to be selected.
%     \item Search Strategy: defined by the naming convention, makeFeatSelControl<search\_strategy>, is used to search the space for all possible feature subsets. There are different search strategies available and our paper utilizes four of these techniques:
%     \begin{enumerate}
%         \item Sequential Forward Search
%         \item Sequential Backward Search
%         \item Genetic Search Algorithm
%         \item Random Search Algorithm
%     \end{enumerate}
%     \item Resampling Strategy: a 10-fold cross validation approach has been implemented to avoid overfitting and a more generalized model output.
% \end{itemize}

% 1. Sequential Forward Search: It is a bottom-up approach algorithm that starts with an empty set and then searches the feature subspace for a feature that can decrease the classification error of the model and adds that feature. This process continues iteratively, until we have a set of features which result in the maximum performance. 

% 2. Sequential Backward Search: It is similar to SFS but reverse. It is a top-down approach in which the algorithm starts with the whole feature set and recursively removes one feature at a time to finally select the minimum required features which gives optimal model performance.

% 3. Genetic Search Algorithm: The Genetic Search Algorithm is derived from Charles Darwin's theory of Natural Selection and it's role in finding the best gene-pairs for a chromosome combination. In our problem, each feature is a gene and the subset of features which give the best performance is our desired chromosome. The algorithm does not rank individual features based on the class variable but tries to find the combination of features which results in the optimal performance of the learning model.

% 4. Random Search Algorithm: The algorithms discussed so far, although effective might result in the learning model being stuck at the local minima and hence the resulting Features selected might not reflect the reality. This is why adding some randomness is always useful in order to avoid local minima. The Random Search Algorithm does the same and searches for feature subsets randomly and measures the model performance through k-fold cross validation(in our case 10-fold cross validation) and repeats it recursively until the optimum result is reached.  

==> Cardiac Cohort Classification based 4D PC-MRI Data/Sections/04-3_classifiers.tex <==
\subsection{Classification Algorithms} %methods
We utilized the following five classification algorithms: 
CART decision tree (DT)~\cite{BreimanEtAl:CART1984}, 
random forest (RF)~\cite{Breiman:RandomForests2001}, 
gradient boosted trees (GBT)~\cite{Friedman:PDP2001},
support vector machine (SVM)~\cite{Boser:SVM1992}, and 
least absolute shrinkage and selection operator (LASSO)~\cite{Friedman:LASSO2010}.

\paragraph*{Decision tree (DT)} A DT classifier recursively divides the data space into a set of non-overlapping subsets based on combinations of feature-value conditions, such as ``IF heart rate $>$ 95 bpm AND max vessel diameter $>$ 35 mm''.
These conditions are constructed in a way that the homogeneity of the target variable within the subsets is reduced. 
Each subset is assigned a class label which is usually the majority class of the training instances within that subset. 
\paragraph*{Tree ensembles}
Random forest (RF) and gradient boosted trees (GBT) classifiers are ensembles of multiple decision trees.
Each base tree casts a vote towards the prediction of the ensemble.  
In a RF base trees are constructed independently from each other, 
whereas trees in a GBT classifier are sequentially added to the ensemble, each of them focusing on areas of the data space where the previously trained trees exhibit high error.

\paragraph*{Support vector machine (SVM)}
In contrast to tree-based models, SVMs also capture non-linear relationships between features and target variable. 
For this purpose, they use a non-linear mapping to expand the feature space of the training set into a higher dimension. 
Within this new feature space, the optimal linear separating hyperplane, i.e., the decision boundary separating the observations from different classes, is detected. 

\paragraph*{Least absolute shrinkage and selection operator (LASSO) classifier}
LASSO is an extension of ordinary least squares linear regression (OLS) whose target function contains an additional regularization term that aims to shrink model coefficients of irrelevant features towards 0. 
Due to its intrinsic feature selection mechanism, LASSO models often are both simpler and more accurate in comparison to OLS~\cite{Hastie:ESL2009}.

% The selection and usefulness of the Feature Selection methods is closely related to the Classification Learning algorithms that were fused with both the Filter and the Wrapper Methods. Our paper tests five classification algorithms in collaboration with each Feature Selection method that has been mentioned earlier. These classification algorithms are as follows:
% \begin{enumerate}
%     \item Decision Tree
%     \item Random Forest
%     \item Support Vector Machine
%     \item Gradient Boosting Machine
%     \item Lasso Regression
% \end{enumerate}

% \textbf{1. Decision Tree:} The Decision Tree algorithm is a supervised top down approach which results in a sequence of decisions taken (features chosen) to come up to a result (class). The depth of the decision tree is built by the various features as nodes depending on criterias such as Information Gain or Gini Index, which depicts how well each Feature is able to classify/distinguish the data into the various classes. So the root node has the highest Information Gain, followed by the other nodes in each layer with decreasing order Information Gain at each level until we finally reach the leaf node or the class node. This results in a sequence/combination of features which when combined together leads to a particular class.

% \textbf{2. Random Forest:} Often the individual output of one Decision Tree might not be good enough to make a decision. Random Forest solves this problem by combining the decision of multiple randomly created Decision Trees to reach to the final decision. The algorithm contains hyperparameters like ntree (number of trees to be built and considered), mtry(number of features on which each tree needs to be built) etc., which can be used for HyperParameter Tuning to obtain the final result. 

% \textbf{3. Support Vector Machines(SVM):} If each feature is considered as one dimension, the SVM algorithm tries to find a Hyperplane almong this N-dimensional space which distinguishes the data distinctly into the various classes. Hyperplanes are decision boundaries which can help in distinguishing the data points into separate class labels. The objective of the SVM algorithm is to find the optimal hyperplane with the maximum margin i.e., the maximal distance between the the data points of each class. The data points which are near the hyperplane are called support vectors as they support in changing the orientation of the hyperplane in a way to distinguish the data points from all the different classes. The dimension of the hyperplane depends on the number of features. For example, if there number of features is 3, the hyperplane is 2 dimensions or a plane. 

% \textbf{4. Gradient Boosting Machine:} Gradient Boosting Algorithm is an Ensemble type of learning algorithm that trains many models in a sequential and additive manner to overcome the shortcomings of weak learning models. The GBM algorithm uses the gradients in a loss function to identify the weak learners. The GBM algorithm allows the user to define a loss function which can determine how well the model is fitting the data points or in other words, are able to distinguish between the data points. This is done by calculating how well the coefficients of the loss function fit the data. The hyperparameters of the GBM algorithm include the "distribution" (bernoullis in our case for classification), "n.trees" which determines the number of weak learning trees that the algorithm will consider, "interaction.depth" which determines the number of features that each tree will have as depth and "shrinkage" which determines the learning rate or the step size for shrinking the importance of each tree after every iteration. 

% \textbf{5. Lasso Regression:} Lasso regression analysis is used for Feature Selection by applying some regularization to normal regression models, in order to increase the classification accuracy as well as the interpretability of the model. The Lasso Regression model adds a regularization term in a way that the model only chooses certain features for prediction, by enforcing the regression coefficients to be less than a particular value, hence enforcing some coefficients to be zero. This helps to avoid overfitting during the overall classification by simplifying the model. This also helps in the interpretability of the model by highlighting the choosing only the correlated set of features.


==> Cardiac Cohort Classification based 4D PC-MRI Data/Sections/04-4_eval.tex <==
\subsection{Evaluation}
We train separate models for each combination of feature selection method (7) and classification algorithm (5), yielding a total of 35 models. 
Hyperparameter selection for the feature selection methods were performed using 10-fold stratified cross-validation. % 
% Since the number of female and male HHV is equal (45), we use accuracy as primary evaluation measure for classification task 3.
We use accuracy as primary evaluation measure for the third classification task which exhibits a balanced class distribution (45 female HHV vs. 45 male HHV). 
Accuracy quantifies the ratio of correctly labeled observations to the total number of observations. 
Due to the class imbalance for the first two classification tasks (90 HHV vs. 22 BAV patients; 30 older HHV vs. 22 BAV patients), we opt for Cohen's kappa, respectively. 
% BAV observations were considered as ``Positive'' class. 
Cohen's kappa is defined as:  
\begin{align}\label{Eq:ScalarVector}
\kappa = \frac {p_{o}-p_{e}}{1-p_{e}}, 
\end{align}
%$\kappa = \frac {p_{o}-p_{e}}{1-p_{e}}$, 
where $p_{o}$ represents accuracy and $p_{e}$ represents the probability for agreement among the vector of true class labels and the class labels assigned by random prediction.
% \textcolor{red}{Kappa value measures the dependence or the inter-rater reliability of the various classes, which means the extent to which the data collectors have assigned the same value to the class variables, given a set of features. It is very robust evaluation measure as it takes into account the probability of a data point being classified as a particular class simply by chance. Again, a higher kappa value means a higher agreement in a particular classification being as such and hence higher confidence in the results. } \textcolor{orange}{@AN: add formula; other question: was kappa also used for tasks 2 and 3 which had a balanced class distribution? if yes, then say which class was set as "positive"}
In addition to accuracy and Cohen's kappa, we report area under the receiver operating characteristic curve (AUC). 
% Cohen's Kappa coefficient (ĸ) was introduced by J. Cohen [44] in 1960 to correlate the measurement of inter-rater reliability. Kappa measures the percentage of agreement between two raters. The formula to calculate Kappa is represented by
A receiver operating characteristic curve visualizes true positive rate (TPR) and false positive rate (FPR) for different prediction thresholds of a binary classifier. 
The area under the ROC curve (AUC) lies between 0 (0\,\% TPR, 100\,\% FPR) and 1 (100\,\% TPR, 0\,\% FPR), where a classifier that makes random predictions achieves an AUC of 0.5. 

% In summary, our approach was to have a combination of each Feature Selection method with every Classification model so explained, to have tally of the performance for each combination and in the end, extract out the best performing combination. For Filtering methods,a FilterWrapper() was created with a fused Feature Selection technique and a Learner. The best Features were extracted initially along with the optimal percentages of Features required for the best results which were then used for the Classification. For Wrapper methods, FeatSelWrapper() was created fused with a search strategy and a Learner which trained and selected the Features simultaneously to give the best output. For all the combinations, there was 10-fold Cross-Validation and Resampling with an iteration of 10. Once a classifcation model was trained with the Training data set, the model was applied to the Test data set to evaluate it's performance. There were 3 evaluation measures which were used:
% \begin{itemize}
%     \item Accuracy: depicts the ratio of all Correctly Predicted samples to the Overall number of samples.
%     \item Area Under the Curve (AUC): AUC is another performance measure for classification which depicts how well a model can separate between each label class. A high value of AUC, maximum being 1, means that the model has very good separability, whereas, AUC of 0 would mean the model has classified each sample wrongly. 
%     \item Kappa: The Kappa value measures the dependence or the inter-rater reliability of the various classes, which means the extent to which the data collectors have assigned the same value to the class variables, given a set of features. It is very robust evaluation measure as it takes into account the probability of a data point being classified as a particular class simply by chance. Again, a higher kappa value means a higher agreement in a particular classification being as such and hence higher confidence in the results. 
    
% In the next section, the results for each evaluation measure for each of these combinations will be discussed.
% \end{itemize}

% 10-fold stratified cross-validation was used for classifier evaluation. 
% In k-fold cross-validation, the data is split into k partitions. 
% Each partition serves once as test set for the model which is trained on the remainder of the partitions.
% Finally, the k performance results are averaged. 


==> Cardiac Cohort Classification based 4D PC-MRI Data/Sections/04_Methods.tex <==
\section{Methods}
\label{sec:framework}
Our data analysis pipeline is depicted in Figure~\ref{fig:pipeline}. %
After extracting the morphologic and hemodynamic features from raw 4D PC-MRI images, we build  separate models for each of three \emph{classification tasks}, i.e., models that distinguish  (1) HHV vs. BAV patients, (2) ``older'' HHV vs. BAV patients and (3) female HHV vs. male HHV.  
For this purpose, we make use of a wide range of feature selection methods and classification algorithms. 
This section describes the main steps of the pipeline, including data prep-processing, feature selection, classification and  evaluation. 
%% ============================================================================

%% ============================================================================
% The data set provided contained 122 samples of patients with 200 features and 1 label column containing 3 classes namely: 1 (depicting "Healthy"), 2 (depicting "Bicuspid Aortic Valve") and 3 (depicting "Tetralogy of Fallot"). The three classification tasks for the project included the tasks to find which features contributed the most towards classifying a patient as Healthy or BAV, to find if Gender has any role in the patient being classified as BAV and atlast to find if Old Healthy patients have the same flow conditions of the heart as the BAV patients.The pipeline for the project hence, required to have three major steps:
% \begin{enumerate}
%     \item Data Pre-Processing
%     \item Cardiological Feature Selection
%     \item Classification and Evaluation
% \end{enumerate}
%% ============================================================================
\input{Sections//04-1_prepro}
\input{Sections//04-2_fs}
\input{Sections//04-3_classifiers}
\input{Sections//04-4_eval}

==> Cardiac Cohort Classification based 4D PC-MRI Data/Sections/05_Results.tex <==
\section{Results}
\label{sec:experiments}
We summarize our classification results in Table~\ref{tab:performance}. 
Table~\ref{tab:hp-tuning} shows the feature selection hyperparameters that were tuned via cross-validation.

\paragraph*{Classification task 1: heart-healthy volunteers (HHV) vs. BAV patients} 
%% ============================================================================
The best model (SFS + RF) achieves Kappa = 0.969 (accuracy = 93.9\%, AUC = 0.796) 
on the test set, cf. Table~\ref{tab:performance}. 
%% ============================================================================
% Three features were selected, (a) \textsf{maxVortexVolumeTime}, (b) \textsf{maxOverallCircumferentialVelocityTime} and (c) \textsf{systolicMaxMeancircumferentialVelocity}.
% \textsf{maxVortexVolumeTime} represents the time point during the heart cycle where the maximum velocity of blood flow occurs in the aorta (in ms; 0 ms = begin of heart cycle). 
% \textsf{maxOverallCircumferentialVelocityTime} depicts the time point during the heart cycle where the maximum circumferential velocity of blood flow occurs in the aorta (in ms). 
% \textsf{systolicMaxMeancircumferentialVelocity} quantifies the maximum of the mean circumferential velocity values of blood flow over all systolic timesteps (in m/s). 
Three features were selected:
\begin{itemize}
\item \textsf{Time-to-Peak-Vorticity}: represents the time point during the heart 
cycle where the overall volume of blood swirling within a vortex in the aorta reaches its peak.
(in ms; 0 ms = begin of heart cycle).
\item \textsf{Time-to-Peak-In-Plane-Velocity}: depicts the time point 
during the heart cycle where the maximum velocity of the in-plane blood 
flow occurs in the aorta (in ms). 
\item \textsf{Peak-Systolic-In-Plane-Mean-Velocity}: quantifies the highest of the mean in-plane blood flow velocities over all planes and systolic timesteps (in m/s).
\end{itemize}
%% ============================================================================

%% ============================================================================
Figure~\ref{fig:plom-pathology-gender}~(a) highlights considerable differences 
between HHV and BAV patients with respect to these three features. 
%% ============================================================================
In particular, BAV patients exhibit a much smaller range in \textsf{Time-to-Peak-Vorticity} 
(min: 130 ms, max: 312 ms) than HHV (min: 0 ms, max: 1573 ms). 
%% ============================================================================
Similarly, whereas all HHV show a \textsf{Peak-Systolic-In-plane-Mean-Velocity} 
of 0.32 m/s or lower, variability within the BAV subgroup is much larger 
(min: 0.12 m/s, max: 0.60 m/s). 
%% ============================================================================

%% ============================================================================
\begin{table}[htb]
\caption{\label{tab:performance} \textbf{Classification results.} 
For each classification task, number of features $d$ and test performance of the five best combinations of feature selection method (FS) and classification algorithm (CA) are depicted. ACC: accuracy.
}
\centering
\begin{tabular}{c@{\hskip 0.20cm}r@{\hskip 0.20cm}l@{\hskip 0.20cm}r@{\hskip 0.20cm}r@{\hskip 0.20cm}r@{\hskip 0.20cm}r}
  \toprule
  \textbf{Classif. task} & \# & \textbf{FS + CA} & $\mathbf{d}$ & \textbf{Kappa} & \textbf{ACC} & \textbf{AUC} \\ 
  \midrule
  \multirowcell{5}{-1-\\HHV vs.\\BAV patients} & 1 & SFS + RF & 3 & \textbf{0.969} & 0.939 & 0.796\\ 
   & 2 & SFS + GBM & 3 & 0.962 & 0.939 & 0.819\\ 
   & 3 & SFS + SVM & 3 & 0.901 & 0.969 & 0.891\\ 
   & 4 & SFS + DT & 2 & 0.639 & 0.878 & 0.935\\ 
   & 5 & CFS + GBM & 19 & 0.796 & 0.939 & 0.898\\
   \midrule
   \multirowcell{5}{-2-\\``older'' HHV vs.\\BAV patients} & 1 & SFS + SVM & 5 & \textbf{1.000} & 1.000 & 1.000\\ 
   & 2 & SFS + RF & 3 & 0.925 & 0.866 & 0.722\\
   & 3 & SFS + DT & 1 & 0.777 & 0.800 & 0.571\\ 
   & 4 & SFS + GBM & 1 & 0.777 & 0.800 & 0.571\\ 
   & 5 & CFS + DT & 6 & 0.705 & 0.866 & 0.833\\
   \midrule
   \multirowcell{5}{-3-\\female HHV vs.\\male HHV} & 1 & SFS + SVM & 3 & 0.384 & \textbf{0.692} & 0.562\\ 
   & 1 & SFS + GBM & 3 & 0.384 & \textbf{0.692} & 0.562\\ 
   & 3 & SFS + RF & 2 & -0.076 & \textbf{0.692} & 0.384\\ 
   & 4 & CFS + GBM & 3 & 0.153 & 0.576 & 0.577\\
   & 5 & SFS + DT & 2 & 0.076 & 0.538 & 0.553\\ 
  \bottomrule
\end{tabular}
\end{table}
%% ============================================================================

%% ============================================================================
\renewcommand{\arraystretch}{1.1}
\begin{table}[htb]
\caption{\label{tab:hp-tuning} 
\textbf{Tuning grid of feature selection (FS) hyperparameters.} 
Values that yield best performance are highlighted in boldface.
}
\centering
% \begin{tabular}{@{\hskip 0.10cm}l@{\hskip 0.20cm}p{4.8cm}@{\hskip 0.20cm}p{2.4cm}}
\begin{tabular}{lp{7cm}l}
  \toprule
  \textbf{FS} & \textbf{Hyperparameter} & \textbf{Candidate values}\\ 
  \midrule
  $\chi^2$ & Relative number of selected features & \{0, $\frac{1}{9}$, $\frac{2}{9}$, $\mathbf{\frac{3}{9}}$, $\ldots$, 1\}\\
  IG & Relative number of selected features & \{0, $\frac{1}{9}$, $\frac{2}{9}$, $\mathbf{\frac{3}{9}}$, $\ldots$, 1\}\\  
  SFS & Minimum improvement in performance when adding a feature $\alpha$ & \{0.005, 0.01, \textbf{0.02}, 0.1\}\\  
  SBS & Maximum decrease in performance when removing a feature $\beta$ & \{$\mathbf{10^{-3}}, 10^{-2}, 10^{-1}$\}\\
  GS & Number of iterations & \{\textbf{10}, 20, 30\}\\  
  GS & Initial number of feature subsets & \{\textbf{10}, 15, 20\}\\  
  RS & Number of iterations & \{10, 50, 100, \textbf{200}\}\\  
  \bottomrule
\end{tabular}
\end{table}
\renewcommand{\arraystretch}{1}

\begin{figure*}[htb]
   \centering
    \makebox[\textwidth]{\makebox[1.4\textwidth]{
       \begin{minipage}{0.7\linewidth}
       \includegraphics[width=\linewidth]{Figures/plom-pathology.pdf}
       \end{minipage}
       \begin{minipage}{0.7\linewidth}
       \includegraphics[width=\linewidth]{Figures/plom-gender.pdf}
       \end{minipage}
    }}
   
   \caption{
     \label{fig:plom-pathology-gender}
     \textbf{Plot matrix for features of best model for classification task 1 (SFS+RF) and 3 (SFS+SVM).}
     Pairwise relationships of the features that were selected for the best feature selection / classification algorithm combination for (a) classification task 1 and (b) classification task 3 are shown. 
     A scatterplot in the lower triangle of the matrix shows the relationship between the feature labeled at the top of the column (x-axis) and the feature labeled at the left of the row (y-axis).  
     Colored lines illustrate the strength of the linear relationship, and labels display the Spearman correlation coefficient ($\rho$). 
     Convex hulls in the scatterplots in the upper triangle of the matrix illustrate the overlap between the two subgroups in the depicted two-dimensional feature space.  
     Histograms on the main diagonal show the distribution of a feature for each target variable. 
    }
\end{figure*}
%% ============================================================================

%% ============================================================================
Visual inspection of the plot matrix in Figure~\ref{fig:plom-pathology-gender}~(a) 
suggests that a simpler model that uses the same feature set is capable to achieve 
high classification performance. 
% The histograms in Figure~\ref{fig:plom-pathology} reveal considerable differences in morphological characteristics between heart-healthy volunteers and BAV patients. %
% For maxVortexVolume, diastolicMaxLeftRotationVolumeRel and systolicMaxMeanPressureInVortexRegion, range and variability in BAV patients is much higher. %
% In fact, the higher homogeneity of heart-healthy volunteers as shown by the scatterplot convex hulls suggests that the relationship between the two cardiac statuses might be represented by an even simpler model with high accuracy. % 
%% ============================================================================
Hence, for each classification task, we used the set of features that led to the 
best classification performance and constructed a decision tree 
% Figure~\ref{fig:decision-trees} shows the decision tree for classification task 1. 
% Only two features are sufficient to achieve excellent discriminative capability 
% (\smalltodo{You mention that the three in figure 6 (a), that two features are sufficient to create a model with high accuracy for the training data. 6 wrong from 22 is around 30\%}
104 out of 112 correctly classified instances). 
%% ============================================================================
The tree in Figure~\ref{fig:decision-trees}~(a) shows descriptions of data regions 
which are representative for either of the two subgroups. 
%% ============================================================================
For example, all 11 subjects with \textsf{Peak-Systolic-In-Plane-Mean-Velocity} 
$\geq$ 0.33 are BAV patients. 
%% ============================================================================
In contrast, 78 out of 82 subjects exhibit a value  $<$ 0.24, cf. leftmost tree 
branch in Figure~\ref{fig:decision-trees}~(a). 
%% ============================================================================
Overall, two features are sufficient to create a model with high accuracy (seven 
misclassifications out of 112 subjects).  
%% ============================================================================

%% ============================================================================
\begin{figure*}[htb]
   \centering
   \makebox[\textwidth]{\makebox[1.3\textwidth]{
     \includegraphics[width=1.3\linewidth]{Figures/decision-trees-cropped.pdf}
   }}
   \caption{
     \label{fig:decision-trees}
    \textbf{Decision trees for each classification task.} 
    Simple decision trees were trained on the full data set using only the subset of features from the best combination of feature selection and classification algorithm. 
    Each terminal node depicts the predicted class label as well as the number of correctly and incorrectly labeled observations. 
    The minimum number of observations in a terminal node was set to 5; the maximum tree depth (number of levels) was set to 4. 
    OHHV: heart healthy volunteers older than 47.
    }
\end{figure*}

\paragraph*{Classification task 2: older HHV vs. BAV patients} 
%% ============================================================================
The best model (SFS + SVM) correctly classifies all 15 test instances 
(Kappa = 1, accuracy = 100\%, AUC = 1). 
%% ============================================================================
% Five features were selected: (a) \textsf{maxMeanAxialVelocity}, (b) \textsf{systolicMaxMeanAxialVelocityTime}, (c) \textsf{diastolicMaxMeanCircumferentialVelocityTime}, (d) \textsf{diastolicMedianRightRotationVolumeRel} and (e) \textsf{maxMeanPressureInVortexRegion}. 
% \textsf{maxMeanAxialVelocity} measures the maximum of the mean velocity values of blood flow that occurs in the aorta over a cardiac cycle (in m/s). 
% \textsf{systolicMaxMeanAxialVelocityTime} indicates the time point during the systole where the maximum of the mean axial velocity values of blood flow occurs in the aorta (in ms). 
% \textsf{diastolicMaxMeanCircumferentialVelocityTime} describes the time point during the diastole where the maximum of the mean axial velocity values of blood flow occurs in the aorta (in ms). 
% \textsf{diastolicMedianRightRotationVolumeRel} represents the median of the volume within the vessel that contains right-handed rotational flow during over all diastolic time steps in relation to the entire vessel volume (in \%). 
% \textsf{maxMeanPressureInVortexRegion} measures the maximum of the mean pressure values over all time steps within the vortex flow regions (in mmHg). 
%% ============================================================================
Five features were selected: 
\begin{itemize}
\item \textsf{Peak-Systolic-Mean-Velocity}: quantifies the highest of the mean through-plane blood flow velocities over all planes and systolic timesteps over a cardiac cycle in the aorta (in m/s). 
%% ============================================================================
\item \textsf{Time-to-Peak-Systolic-Through-Plane-Mean-Velocity}: indicates the time point during 
the systole where the mean through-plane velocity over all planes' peaks (in ms). 
%% ============================================================================
\item \textsf{Time-to-Peak-Diastolic-In-Plane-Mean-Velocity}: describes the time point during 
the diastole where the mean in-plane velocity over all planes' peaks (in ms).
%% ============================================================================
\item \textsf{Diastolic-Median-Right-Rotation-Volume-Rel}: represents the median of 
the volume within the vessel that contains right-handed rotational flow during 
over all diastolic time steps in relation to the entire vessel volume (in \%). 
%% ============================================================================
\item \textsf{Peak-Mean-Vorticity-Pressure}: measures the highest of the mean 
pressure value withing vortex regions over all time steps (in mmHg). 
\end{itemize}
%% ============================================================================

%% ============================================================================
Histograms and convex hulls in Figure~\ref{fig:plom-ohhv_bav} demonstrate large 
difference in the distribution of \textsf{diastolic-Median-Right-Rotation-Volume-Rel} 
between older HHV (mean: 0.51 $\pm$ standard deviation: 0.01) and BAV patients 
(0.61 $\pm$ 0.09). 
%% ============================================================================
The first node of the decision tree depicted in Figure~\ref{fig:decision-trees}~(b), which is trained on the five above features, confirms the high association between \textsf{diastolic-Median-Right-Rotation-Volume-Rel} and subgroup membership. 
More specifically, a value greater equal than 53\% is characteristic for BAV 
patients (17 out of 22 subjects). 
%% ============================================================================
Overall, the ``decision stump'' (only one split) in Figure~\ref{fig:decision-trees}~(b) 
correctly assigns 45 out of 52 subjects to their respective subgroup. 

\begin{figure*}[h!]
   \centering
%   \includegraphics[width=\linewidth]{Figures/plom-ohhv_bav.pdf}
   \includegraphics[width=\linewidth]{Figures/plom-ohhv_bav.pdf}
   \caption{
     \label{fig:plom-ohhv_bav}
     \textbf{Plot matrix for features of best model of classification task 2 (SFS+SVM).}
     Pairwise relationships of the features that were selected for the best feature selection / classification algorithm combination of classification task 2 (sequential forward selection + support vector machine) are shown. See Figure~\ref{fig:plom-pathology-gender} for a description.
    }
\end{figure*}

\paragraph*{Classification task 3: female vs. male HHV}
The combination of SFS and RF achieves best generalization performance (accuracy = 69.2\%, Kappa = 0.384, AUC = 0.562), cf. Table~\ref{tab:performance}. 
Just as with the first classification task, three features were selected: 
% (a) \textsf{maxOverallVelocity}, 
% (b) \textsf{systolicMaxOverallVelocityQ99} and 
% (c) \textsf{distolicMaxOverallAxialVelocityTime}. 
% \textsf{maxOverallVelocity} measures the maximum velocity of blood flow that occurs in the aorta over a cardiac cycle (in m/s). 
% \textsf{systolicMaxOverallVelocityQ99} depicts the maximum velocity of blood flow (from the 99.5\% quantile range) that occurs in the aorta during the systolic phase of the cardiac cycle (in m/s).
% \textsf{diastolicMaxOverallAxialVelocityTime} represents the time point during the diastole where the maximum axial velocity of blood flow occurs in the aorta (in ms; 0 ms = begin of heart cycle). 
%% ============================================================================
\begin{itemize}
\item \textsf{Peak-Velocity}: measures the maximum velocity of blood flow 
that occurs in the aorta over a cardiac cycle (in m/s). 
%% ============================================================================
\item \textsf{Peak-Systolic-VelocityQ99} depicts the maximum velocity of 
blood flow (taken from the 99.5\% quantile range to discard outliers due to noise) that occurs in the aorta during the 
systolic phase of the cardiac cycle (in m/s). 
%% ============================================================================
\item \textsf{Time-to-Peak-Diastolic-Through-Plane-Velocity} represents the time point 
during the diastole where velocity of the through-plane blood flow peaks in any of the planes in 
the aorta (in ms; 0 ms = begin of heart cycle). 
\end{itemize}
%% ============================================================================

%% ============================================================================
Although these three features yield the best model, the plot matrix in Figure~\ref{fig:plom-pathology-gender}~(b) shows that female and male HHV have quite similar value distributions. 
Consequently, the decision tree trained on \textsf{Peak-Velocity}, \textsf{Peak-Systolic-VelocityQ99} and \textsf{Time-to-Peak-Diastolic-Through-Plane-Velocity} (Figure~\ref{fig:decision-trees}~(c)) is more complex than the other trees and has only mediocre classification performance, as one third of the subjects are misclassified. 

% \begin{figure*}[htb]
%   \centering
%   \includegraphics[width=.7\linewidth]{Figures/plom-gender.pdf}
%   \caption{
%      \label{fig:plom-gender}
%      \textbf{Plot matrix for features of best model of classification task 3 (SFS+SVM).}
%      Pairwise relationships of the features that were selected for the best feature selection / classification algorithm combination of classification task 3 (sequential forward selection + support vector machine) are shown. See Figure~\ref{fig:plom-pathology} for a description.
%     }
% \end{figure*}

% As discussed previously, there were three distinct classification tasks addressed in this paper. The results for the first Classification task i.e to distinguish between Healthy and BAV patients was found to be best given by the Sequential Forward Feature Selection method with a Support Vector Machine as the classifier. It gives an Accuracy of 96.9\%, an AUC of 0.901 and a Kappa value of 0.891 for the Test Set with just three features, namely:
% \begin{enumerate}
%     \item maxVortexVolume
%     \item diastolicMaxLeftRotationVolumeRel
%     \item systolicMaxMeanPressureInVortexRegion
% \end{enumerate}
% The high value of Accuracy testifies the fact that the model is able to correctly classify samples which it has not seen before with these features. The high AUC and Kappa values depict a high confidence for the results from the model or in other words, depicts how confident the model is in the results for the classification. The second and third best result were also given by the Sequential Forward Feature Selection along with Gradient Boosting Machine and Random Forest as classifiers respectively. The features obtained by these algorithms are as follows: 

% For GBM:
% \begin{enumerate}
%     \item maxVortexVolumeTime              
%     \item diastolicMaxVortexVolumeTime     
%     \item medianMeanPressureInVortexRegion
% \end{enumerate}

% For Random Forest:
% \begin{enumerate}
%     \item maxVortexVolumeTime                   
%     \item maxOverallCircumferentialVelocityTime  
%     \item systolicMaxMeancircumferentialVelocity
% \end{enumerate}

% As the results clearly depict, the feature maxVortexVolume and it's variation maxVortexVolumeTime is an important feature for the classification of the patients into Healthy and BAV. A simple algorithm like a Decision Tree classifier also was able to achieve an Accuracy of 81.8\% with just two features namely, maxVortexVolume and diastolicMaxMeanAxialVelocityTime. On plotting the Decision Tree it was seen that 13\% of the data was already classified as BAV if the maxVortexVolume of the patient was seen to be less than 64. The patients with maxVortexVolume greater or equal to 64 were further analyzed with the feature diastolicMaxMeanAxialVelocityTime. 51\% of these patients had a diastolicMaxMeanAxialVelocityTime of more than 504 and were immediately classified as Healthy. Hence, this Decision Tree analysis further solidifies the claim that maxVortexVolume is a very important feature in recognition of BAV conditions for patients. 

% The second classification task included checking if Gender played any role in deciding the health condition of a patient. The results were based on 45 healthy males and females to check if the classifier was able to distinguish between the genders based on the Features extracted by the Feature Selection Techniques. The optimal combination for the classification was obtained by Sequential Feature Selection method with SVM Classifier as well as the GBM Classifier which both resulted in a mere 69.2\% Accuracy and an AUC and Kappa of 0.562 and 0.384 respectively. The features selected were "maxOverallVelocity", "systolicMaxOverallVelocityQ99", and "diastolicMaxOverallAxialVelocityTime". The Decision Tree was next with two features selected ("medianDiameter" and "diastolicMaxMeanAxialVelocity") and an Accuracy of 53.8\%. It was also seen that as the number of Features selected for different Feature Selection techniques increased, the accuracy increased only to a maximum of 80.7\% with thirty five features but the rate of misclassifications was still very high for a data set of ninety data points. The low Accuracy and confidence levels of the classifcation models suggest that the model was not able to distinguish between Healthy Males and Females based on the Features extracted, further verifying the hypothesis that there is no difference between the flow conditions of Healthy Males and Healthy Females and as such Gender does not play a role in determining the BAV characteristic of a patient.

% The third classification task was to understand if older Healthy patients had similar flow conditions to BAV patients. For this analysis was done on two subgroups of data: Healthy patients above 47 years of age and all BAV patients to see if the model would misclassify any Healthy patients as BAV. If this number of misclassifications was high and belonged to the older age group, it would mean that the flow conditions was not different between the older Healthy patients and the BAV group, leading to the model not being able to distinguish between the two classes. The results however showed otherwise, as with even small number of features, the accuracy obtained was pretty high. The best results were again for Sequential Forward Feature Selection with Random Forest Classifier. Intially the Accuracy obtained with the age parameter as a feature was always more than 90\% and the Decision Tree was able to classify 100\% of the data based on just the Age feature. But as there was already a bias associated with the Age during the initial data extraction, the Age parameter was removed to check if the model still performs well enough. The Accuracy obtained with three selected features(maxVortexVolumeTime,systolicMaxVortexVolume,
% diastolicMedianRightRotationVolumeRel) was 86.6\% with a AUC of 0.722 and Kappa of 0.925 depicting very high confidence, even with the Age parameter removed. The GBM and Decision Tree was also able to achieve 80\% Accuracy levels with high confidence with just one feature each (diastolicMedianRightRotationVolumeRel<0.53 is Healthy and rest are BAV). This analysis rejects our hypothesis that the older Healthy patients have the same flow conditions as the BAV patients.  




  


==> Cardiac Cohort Classification based 4D PC-MRI Data/Sections/06_Discussion.tex <==
\section{Discussion}
\label{sec:disc}
%% ============================================================================
Our classification results suggest substantial differences in flow characteristics 
of the aorta between HHV and bicuspid aortic valve (BAV) patients. 
%% ============================================================================
For several of the features, BAV patients exhibit higher variation and higher 
value ranges. 
%% ============================================================================
To proof the validity of our models, we discussed the results with a radiologist 
(co-author), specialized in cardiac imaging with 23 years of work experience. 
%% ============================================================================
He also provided the data sets. 
%% ============================================================================

%% ============================================================================
The possible aortic valve stenosis due to the altered valve morphology 
in BAV patients means that the heart must exert more force to open the valve and 
pump the blood further because of this resistance. 
%% ============================================================================
Consequently, the flow velocity increases significantly compared to healthy 
individuals, especially during systole. 
%% ============================================================================
The strong increase in flow velocity favors the formation of vortical blood flow 
within the aorta. 
%% ============================================================================
As a result, the forward movement of the flow along the centerline decreases and 
there is more flow that rotates within a plane. 
%% ============================================================================
This is also reflected in the classification results for the first task. 
%% ============================================================================

%% ============================================================================
The parameter \textsf{Peak-Systolic-In-Plane-Mean-Velocity} represents the 
velocity of flow in a plane. 
%% ============================================================================
In HHV it is less than 30 cm/min and the average flow velocity is 1.5 m/sec. 
%% ============================================================================
Accordingly, the velocity of flow in a plane in BAV patients is at least one 
third of the average flow velocity, which is a very high value. 
%% ============================================================================
These circumstances explain the good initial separation of HHV and BAV patients 
based on \textsf{Peak-Systolic-In-Plane-Mean-Velocity}. 
%% ============================================================================
The second parameter \textsf{Time-to-Peak-In-Plane-Velocity} measures 
the time of maximum flow velocity in one plane. 
%% ============================================================================
The radiologist assumes that this is the corresponding time for 
the \textsf{Peak-Systolic-In-Plane-Mean-Velocity}. 
%% ============================================================================
Due to the high flow velocity in BAV patients, vortical flow occurs earlier 
during the cardiac cycle and therefore the \textsf{Time-to-Peak-In-Plane-Velocity} 
occurs earlier than in healthy volunteers. 
%% ============================================================================
Nevertheless, the radiologist was positively surprised that 
only two parameters allow a good separation of both classes. 
He emphasized 
that determining the corresponding threshold values 
is of paramount importance 
%as elementary important 
to support the diagnosis of CVDs. 
%% ============================================================================

%% ============================================================================
With respect to our second research question, we could not confirm that older HHV show similar flow characteristics as BAV patients in the current data set.
% \todo[inline,caption={}]{
% \begin{itemize}
%     \item Hypothesis in general can just be rejected, not really confirmed. Maybe the authors should review their formulations such that it is more accurate. For example, when they discuss whether an hypothesis was rejected and confirmed. From a formal point of view I think they cannot really say that without some question marks.
%     \item I am a bit confused about the statements in the discussion and conclusions around the 2nd hypothesis. The 2nd hypothesis is "rejected" since there is difference found between the groups which the hypothesis says should be equal. You mention that "we conclude that our approach to extract interpretable features for the diagnosis of BAV patients is sensible" what do you mean with sensible? technically sound? sensible for what?
%     \item The paragraph about hypothesis two in the conclusions is confusing to me... you say "you were able to confirm the hypothesis " which I think is not true. The hypothesis is formulated there with "whether there is..."I would say this is not a good hypothesis formulation.
% \end{itemize}
% }
%% ============================================================================
The parameter \textsf{Diastolic-Median-Right-Rotation-Volume-Rel} allows a reliable 
separation of both groups with 7 out of 45 data sets being misclassified. 
%% ============================================================================
In HHV, only during systole slight vortical flow occurs, whereas during diastole 
hardly any vortical flow occurs because the aortic valve is completely closed. 
%% ============================================================================
This is also the case in older subjects. 
%% ============================================================================
BAV patients on the other hand show increasing vortical flow, also during diastole, 
which is why a differentiation of both groups was possible here. 
%% ============================================================================
Since the best models have excellent performance while requiring only three to 
five features, we conclude that our approach to extract interpretable features 
for the diagnosis of BAV patients is sensible. 
%% ============================================================================

%% ============================================================================
From the performance of the classifiers for the 
% \smalltodo{- Feature selection is sensitive also has the problem that you might actually be removing the features that make the difference. It would be good to comment on that specially for the third hypothesis}
third classification task, we 
infer that, although there are minor differences between female and male HHV, 
morphological and hemodynamic characteristics alone are not sufficient to distinguish 
between genders with high accuracy. 
%% ============================================================================
This also met the expectations of our radiologist. 
%% ============================================================================
Although on average men have a larger heart and blood volume than women, this 
does not significantly affect the derived morphological and hemodynamic characteristics. 
%% ============================================================================
Nevertheless, such a detailed analysis of HHV is important to derive 
normal values and thus reliably detect abnormal characteristics. 
%% ============================================================================

%% ============================================================================
Although we consider our results to be promising, there are some limitations and 
room for improvement. 
%% ============================================================================
First, our data set might be subject to a selection bias. 
%% ============================================================================
The HHV group includes only volunteers who are at least 18 and at most 65 years 
old. 
%% ============================================================================
Older volunteers were excluded because they had already shown an enlargement 
of the aortic diameter which, although not yet in need of treatment, deviated 
from a physiological morphology. 
%% ============================================================================
Accordingly, our calculated age limit of 47 years for classifying older HHV and 
BAV patients was rather low, which might explain the good separability. 
%% ============================================================================
Regarding BAV cases only patients over 18 years were considered. 
%% ============================================================================
Children were therefore not included in the data collective, although it would 
be an interesting question whether children could be separated as well as adult 
BAV patients from HHV. 
%% ============================================================================
In addition, no distinction was made in the BAV patients regarding 
pronounced secondary diseases, aortic valve stenosis and aortic valve insufficiency. 
%% ============================================================================
This could also influence the classification. 
%% ============================================================================

We used the Information Gain measure to determine the cutoff value of 47 years to divide the subjects into two subsets based on age. 
Alternatively, we could have also tested multiple thresholds to ultimately choose the cutoff value which yields best classification performance.   
However, a study involving coronary artery disease patients~\cite{Kuecherer1988} also showed that patients of ca. 50 years of age and older had similar ventricular diastolic filling to the control group, while there were larger differences between groups in younger subjects.

While the decision trees in Figure~\ref{fig:decision-trees} illustrate the protectiveness of some of the extracted features towards the target variables, 
they should be interpreted with caution, as they were trained on the total data set, and thus, have limited generalization value.

%% ============================================================================
In addition, our holdout evaluation might be subject to high variability of the 
generalization error estimates, especially for classification task 2 where the test 
set contains only 15 observations (ca. 30\%). 
%% ============================================================================
To assess the performance gain of our feature selection step, we also consider to train classifiers using all available features. 
We did not attempt this here, as the size of the feature space would have been ca. twice as large as the size of the data set and the performance estimates would have been even more prone to the effects of overfitting.
%% ============================================================================
In future, we would like to expand our data analysis pipeline with a nested-cross 
validation scheme that involves tuning of feature selection hyperparameters in 
the inner loops and calculation of generalization performance on multiple outer folds, 
thus reducing variability of the performance estimates. 
%% ============================================================================
Apart from parameters of the feature selection methods, we will consider also 
tuning classifier hyperparameters to further improve model performance. 
%% ============================================================================


% morph. + hemodyn. parameters alone are not suff to build a robust model to determine the gender of the subject
% limitation: small number of test instances
% mischung us rel und abs

% maxVortexVolume: the maximum amount of vortical flow that occurs in the aorta over a cardiac cycle, derived from regions with negative relative pressure. Unit: ml
% diastolicMaxLeftRotationVolumeRel: Maximum of the volume within the vessel that contains left-handed rotational flow over all systolic time steps in relation to the entire vessel volume. Unit: %
% systolicMaxMeanPressureInVortexRegion: the maximum of the mean pressure values over all systolic time steps within the vortex flow regions. Unit: mmHg
% maxVortexVolumeTime: The time point during the heart cycle (0ms = begin of heart cycle) where the maximum velocity of blood flow occurs in the aorta. Unit: ms
% systolicMaxVortexVolume: the maximum amount of vortical flow that occurs in the aorta during the systolic phase of the cardiac cycle. Unit: ml
% diastolicMedianRightRotationVolumeRel: Median of the volume within the vessel that contains right-handed rotational flow during over all diastolic time steps in relation to the entire vessel volume. Unit: %
% maxOverallVelocity: the maximum velocity of blood flow that occurs in the aorta over a cardiac cycle Unit: m/s
% systolicMaxOverallVelocityQ99: the maximum velocity of blood flow (from the 99.5 quartile range) that occurs in the aorta during the systolic phase of the cardiac cycle Unit: m/s
% diastolicMaxOverallAxialVelocityTime: The time point during the diastole (0ms = begin of heart cycle) where the maximum axial velocity of blood flow occurs in the aorta. Unit: ms

% maxOverallCircumferentialVelocityTime: The time point during the heart cycle where the maximum circumferential velocity of blood flow occurs in the aorta. Unit: ms

% systolicMaxMeancircumferentialVelocity: Maximum of the mean circumferential velocity values of blood flow over all systolic timesteps. Unit: m/s

% maxMeanAxialVelocity: the maximum of the mean velocity values of blood flow that occurs in the aorta over a cardiac cycle Unit: m/s

% systolicMaxMeanAxialVelocityTime: The time point during the systole where the maximum of the mean axial velocity values of blood flow occurs in the aorta. Unit: ms

% distolicMaxMeanCircumferentialVelocityTime: The time point during the diastole where the maximum of the mean axial velocity values of blood flow occurs in the aorta. Unit: ms

% maxMeanPressureInVortexRegion:  the maximum of the mean pressure values over all time steps within the vortex flow regions. Unit: mmHg

==> Cardiac Cohort Classification based 4D PC-MRI Data/Sections/07_Conclusion.tex <==
\section{Conclusion and Future Work}
\label{sec:con}
%% ============================================================================
We present a data analysis pipeline for the classification of BAV patients vs. HHV. 
%% ============================================================================
Therefore, we initially extract a large number of morphological and hemodynamic 
features from 4D PC-MRI data sets. 
%% ============================================================================
We integrated various feature selection methods with classifier training to 
reduce the number of features, aiming to build accurate yet parsimonious classification 
models. 
%% ============================================================================
Finally, we constructed decision trees using the subset of features found to 
achieve best classification performance. 
%% ============================================================================
Our results show differences between BAV patients and HHV with respect to 
hemodynamics, such as the higher blood flow velocity in BAV patients. 
%% ============================================================================
Furthermore, we applied our pipeline to two other classification tasks. 
%% ============================================================================
First, we investigated the question whether there are morphological and 
hemodynamic differences between \emph{``older''} HHV and BAV patients, which was 
derived from the observation that the heart function seems to decrease with age. 
%% ============================================================================
We were able to confirm this based on the high performance of the classifiers, 
although our results must be verified on another independent data set. 
%% ============================================================================
Second, we trained a model that distinguishes between female and male HHV based 
on the extracted features. 
%% ============================================================================
Although our models are more competitive than random guessing, we did not identify 
one or a combination of features that are capable to predict gender very accurately. 
%% ============================================================================

%% ============================================================================
In the future, we plan to extend our pipeline to other pathologies, e.g., diseases 
of other heart vessels, such as the Tetralogy of Fallot, which primarily show 
changes in the pulmonary artery. 
%% ============================================================================
This may contribute to improve the diagnostic workflow.
%% ============================================================================
Furthermore, we want to expand our data collection to include more older 
heart-healthy volunteers (60 years of age and older) and repeat the second classification 
task to check whether healthy aging people show similar characteristics to BAV 
patients.
%% ============================================================================
Moreover, we plan to evaluate the treatment success, e.g., after an aortic valve 
replacement, to check whether the flow normalizes after surgery. 
%% ============================================================================
For this purpose, we want to apply our trained models to new treated cases and 
check if they are classified as heart-healthy. 
%% ============================================================================
This would provide insights into whether the flow returns to normal after the 
insertion of an artificial heart valve.  
